A Multiversion Programming Inspired Approach to Detecting Audio Adversarial Examples

Adversarial examples (AEs) are crafted by adding human-imperceptible perturbations to inputs such that a machine-learning based classifier incorrectly labels them. They have become a severe threat to the trustworthiness of machine learning. While AEs in the image domain have been well studied, audio AEs are less investigated. Recently, multiple techniques are proposed to generate audio AEs, which makes countermeasures against them an urgent task. Our experiments show that, given an AE, the transcription results by different Automatic Speech Recognition (ASR) systems differ significantly, as they use different architectures, parameters, and training datasets. Inspired by Multiversion Programming, we propose a novel audio AE detection approach, which utilizes multiple off-the-shelf ASR systems to determine whether an audio input is an AE. The evaluation shows that the detection achieves accuracies over 98.6%.

==> Architecture_Diversity.tex <==
\section{Diverse ASRs}
\label{Architecture_Diversity}
Yu and Li \cite{yu2017recent} summarized the recent progress in deep-learning based ASR acoustic models, where both recurrent neural network (RNN) and convolutional neural network (CNN) come to play as parts of deep neural networks. Standard RNN could capture sequence history in its internal states, but can only be effective for short-range sequence due to its intrinsic issue of exploding and vanishing gradients. This issue is resolved by the introduction of long short-term memory (LSTM) RNN \cite{Hochreiter:1997:LSM}, which outperforms RNNs on a variety of ASR tasks \cite{DBLP:conf/icassp/GravesMH13,sak2014LSTM,DBLP:journals/corr/LiW14a}. As to CNNs, its inherent translational invariability facilitates the exploitation of variable-length contextual information in input speech. The first CNN model proposed for ASRs is time delay neural network \cite{DBLP:journals/nn/LangWH90} that applies multiple CNN layers. Later, several studies \cite{DBLP:conf/interspeech/Abdel-HamidDY13,DBLP:conf/icassp/Toth15,DBLP:journals/corr/SercuG16a} combine CNN and Hidden-Markov Model to create hybrid models that are more robust against vocal-tract-length variability between different speakers.
But there is \emph{no} single uniform structure used across all ASRs.

In addition to several well-known ASR systems, multiple companies have independently 
developed their own ASRs, such as \emph{Google Now}, \emph{Apple Siri} and \emph{Microsoft Cortana}. In our system, we use \emph{DeepSpeech}, \emph{Google Cloud Speech}, and \emph{Amazon Transcribe}. \emph{DeepSpeech} is an end-to-end speech recognition software open-sourced by Mozilla. Its first version \cite{DBLP:journals/corr/HannunCCCDEPSSCN14} uses a five-layers neural network where the fourth layer is a RNN layer, while the second version \cite{amodei2016deep} contains a mix of CNN and RNN layers. Our experiments used the first version, as the second version was not publicly 
available at the time of our experiment. 
Unlike \emph{DeepSpeech}, the DNN behind Google Cloud Speech is a LSTM-based RNN according to the source \cite{OnlineRef:Google_AI_Blog_NNs_behind_GCS}. Each memory block in Google's LSTM network \cite{sak2014LSTM} is a standard LSTM memory block with an added recurrent projection layer. This design enables the model's memory to be increased independently from the output layer and recurrent connections. No public information about the internal
details of \emph{Amazon Transcribe} is available. 

%It is worth nothing that even black-box AE generation methods~\cite{DBLP:journals/corr/abs-1805-07820,alzantot2018did} need
%the \emph{logits} outputs of a network to run the algorithms, while that information
%is not provided by many proprietary systems, such as \emph{Google Cloud Speech} and \emph{Amazon Transcribe}. 
%This makes the generation of AEs effective on these systems much more difficult,
%if not impossible. 

In short, existing ASR systems are diverse with regard to architectures, parameters and training datasets. 
Compared to opensourced systems, propriety ASR systems provide little information that can be exploited by attackers. 
Given the diversity of ASR systems (and proprietary networks), it is unclear how
to propose a generic AE generation method that can simultaneously mislead all of them. 

%Not only that it is difficult to generate transferable AEs, but it is also
%difficult to build a generic AE generation

%This reminds us of Multiversion Programming, 
%a method in software engineering where multiple functionally equivalent programs are
%independently developed from the same specification, such that an attack input that
%compromises one of them are ineffective on other programs.

==> old-system-design.tex <==
\section{System Design}\label{sec:systemdesign}



\begin{figure}[t]
	\centering
	\includegraphics[width=\linewidth]{./figures/Overview_of_AE_Detection_System.png}
	\caption{Overview of the proposed detection system.}
	\label{fig:system_overview}
	\vspace{-10pt}
\end{figure}



In software engineering, \emph{multi-version programming} (MVP) is an approach that \emph{independently} develops multiple software programs 
based on the same specification, %MVP introduces redundancy of software functionalities in order to improve reliability of software operations. 
such that an exploit that compromises one program probably fails on other programs. 
This inspires us to propose a system design that runs multiple ASRs in parallel to detect audio AEs
as shown in Figure \ref{fig:system_overview}, where the \emph{target} ASR is the system targeted by
the adversary (e.g., the speech recognition system at a smart home) and  \emph{auxiliary} ASRs are models
different from the target ASR.

\begin{table}[t]
%\vspace{-3pt}
                \centering
                \caption{Recognition results of an AE by multiple ASRs: the host transcription is ``\emph{I wish you wouldn't}'', while the embedded text is ``\emph{a sight for sore eyes}''.}
                \vspace{3pt}
                \label{Table:Transcriptions_of_an_AE}
                \begin{tabular}{cl}
                                \hline
                                ASR & Transcribed Text \\ \hline
                                DeepSpeech v0.1.0 & \emph{A sight for sore eyes} \\
                                DeepSpeech v0.1.1 & \emph{I wish you live} \\
                                Google Cloud Speech & \emph{I wish you wouldn't}. \\
                                Amazon Transcribe & \emph{I wish you wouldn't}. \\ \hline
                \end{tabular}
                \vspace{-3pt}
\end{table}

The intuition behind this design is that different ASRs 
%or even the same DNN model with different configurations 
can be regarded as ``independently developed programs'' in MVP.
Since they follow the same specification, that is, to covert audios into texts,
given a benign sample, they should output very similar recognition results.
On the other hand, an audio AE can be regarded as an ``exploit'', and cannot fool all ASRs as verified in
Section~\ref{sec:transferability}.
%could result into a significant mismatching of speech recognition results on an input AE. 
%We believe the intuition holds since targeted audio AEs produced by existing approaches fails to transfer. 
Thus, the recognition result by the target ASR differs \emph{significantly} from those by the auxiliary ASRs.
Table~\ref{Table:Transcriptions_of_an_AE} shows a typical example, which can only fool one ASR and fails on others. 


The system works as follows: 1) the target and auxiliary ASRs simultaneously conduct speech-to-text conversion, 2) then the transcriptions are used to calculate similarity score(s), which are passed into a binary classifier to determine whether the input audio is adversarial. 




Similarity scores are calculated in two steps. First, each transcription is converted into its phonetic-encoding representation. Phonetic encoding converts a word to the representation of its pronunciation \cite{OnlineRef:PhoneticEncoding}. This helps handle variations between ASRs, as they may output different words
for similar pronunciations. The validity of using phonetic encoding will be demonstrated in Section \ref{subsection:discussion_similarity_metrics}. Second, for each auxiliary ASR, a similarity score is calculated
to measure the similarity between the text recognized by the target ASR and that by the auxiliary ASR. 
We adopt the Jaro-Winkler distance method \cite{OnlineRef:Jaro-Winkler-Similarity} to calculate the similarity score
(see Section~\ref{subsection:discussion_similarity_metrics} ). It gives a value between 0 and 1, where 0 indicates totally dissimilar and 1 very similar.

